Enhancing Performance of Explainable AI Models with Constrained Concept Refinement

The trade-off between accuracy and interpretability has long been a challenge in machine learning (ML). This tension is particularly significant for emerging interpretable-by-design methods, which aim to redesign ML algorithms for trustworthy interpretability but often sacrifice accuracy in the process. In this paper, we address this gap by investigating the impact of deviations in concept representations-an essential component of interpretable models-on prediction performance and propose a novel framework to mitigate these effects. The framework builds on the principle of optimizing concept embeddings under constraints that preserve interpretability. Using a generative model as a test-bed, we rigorously prove that our algorithm achieves zero loss while progressively enhancing the interpretability of the resulting model. Additionally, we evaluate the practical performance of our proposed framework in generating explainable predictions for image classification tasks across various benchmarks. Compared to existing explainable methods, our approach not only improves prediction accuracy while preserving model interpretability across various large-scale benchmarks but also achieves this with significantly lower computational cost.

==> main_text/introduction_old.tex <==
Machine learning algorithms have long grappled with a critical trade-off: models designed for interpretability often sacrifice performance, while high-performing models lack transparency. Some representatives for the former class of algorithms include linear regressions and decision trees, where predictions made by the algorithm can be easily comprehended through the weights of some key parameters. While on the other end of the spectrum, models like deep neural networks are difficult to understand as the number of parameters involved is huge. The situation is even more true for the state of the art models like large language models. There are several methods proposed to draw interpretability from the second category of the models \cite{baehrens2010explain, simonyan2013deep, zeiler2014visualizing, shrikumar2017learning, selvaraju2017grad, smilkov2017smoothgrad, kolek2020rate, subramanya2019fooling}. However, all of these methods adopt a post-hoc approach which mostly uses sensitivity analysis to locate the key weights in a model that affect final predictions. As a result, there are no guarantees that these methods can provide an explanation for every predictions made by the model, nor guarantees that they are trustworthy \cite{adebayo2018sanity, rudin2019stop, kindermans2019reliability, ghorbani2019interpretation, slack2020fooling}. Consequently, people turn to models that are \textit{interpretable by design}, where each prediction made by the model is coupled with a self-generated explanation. Ideally, the explanation provided here should be closely related to the generation of prediction and also intuitive or interpretable for humans. One of the most representative work is Concept Bottleneck Models(CBM,\cite{koh2020concept}), which first learn a mapping from raw input to an intermediate set of human-specified concepts and then make the prediction using the learned score of this concept sets. The training of this architecture requires datasets with concept score explicitly labeled. Several similar models\cite{yuksekgonul2022post, oikarinen2023label} has been proposed to replace the concept-learning module with multi-modal models like CLIP. In \cite{chattopadhyay2022interpretable}, authors proposed to learn the true label with a decision tree structure where each decision is made based on taking some human-defined concept embeddings and previous decision history as input. The method, termed as V-IP, is easy to interpret by humans and \cite{chattopadhyay2024information} proposed its advanced version with significantly less computational cost. A high level summarization for some of the aforementioned methods are given by \Cref{fig:flowchart}: they first generate embeddings for data input like images and concept input (either given by human experts or ChatGPT), then feed them into an interpretable model to generate the prediction. The interpretable model should be simple and intuitive enough for human to derive comprehension and the training process focuses on updating the parameters for the model itself. Concept embeddings actually play an important role in the framework: not only do they influence the process of generating predictions, the corresponding weights to these embeddings are also the source of interpretability for the whole algorithms. There are mainly two types of concept encoders which takes human or ChatGPT specified concepts and turn them into embeddings: one is trained from scratch using datasets with concept properties labeled like \cite{koh2020concept,oikarinen2023label}; the other type utilize the pre-trained encoders like CLIP \cite{yuksekgonul2022post,chattopadhyay2024information}. For the first type of encoder, issues have been raised about its ambiguity \cite{margeloiu2021concept,watson2022conceptual,kim2023probabilistic,marconato2023interpretability}, fragility \cite{furby2024can} and low accuracy \cite{zarlenga2022concept,chowdhury2024adacbm}. For pre-trained encoders like CLIP, challenges with respect to domain adaptation \cite{shao2023investigating, gondal2024domain, feng2024rethinking, wang2024attention}, bias in the pre-training data \cite{hamidieh2024identifying} and sensitivity to encoding issues\cite{ranjan2024unveiling} have also been revealed in the recent literature. There have been some efforts to mitigate the challenge of unreliable concept embeddings. \cite{sawada2022concept} proposed to learn an additional unsupervised concept module to increase the expressiveness of the concept set. \cite{yuksekgonul2022post} proposed to directly train a residual learning module to work parallel with concept encoder to increase accuracy. \cite{zarlenga2022concept} proposed to learn two concept embeddings for each concept and \cite{chowdhury2024adacbm} proposed to add a special data encoder to deal with the domain shift. All the methods mentioned above are trying to increase the prediction accuracy by adding more black box learning modules to the model. Even though these attempts are good reflections for the trade-off between performance and interpretability, it is yet unknown if adding more opaque learning layers is the most cost-efficient way to redeem accuracy. Another important aspect that has been largely neglected by the community is the theoretical guarantees that come along with the new algorithms. Unlike deep and large models, \textit{interpretable by design} models mostly adopt simple architectures for transparency, which should be amenable to theoretical analysis. Yet all the works mentioned here cannot provide any theoretical guarantees, which is especially of interest in problems that are safety critical like medical imaging \cite{barragan2021artificial} and autonomous vehicles \cite{bensalem2023indeed}. To sum up, it is still an open challenge to find a theoretically reliable and practically competent model that maintain interpretability.

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figs/flowchart.png}
    \caption{The red arrows and boxes represent the back-propagation training process for classic explainable AI models. In this paper, we propose to extend the training process to refine concept embeddings with constraints on its deviation from the initial embeddings, indicated by green arrows and circles.}
    \label{fig:flowchart}
\end{figure}

In this paper, we propose a framework termed as \textit{Constrained Concept Refinement} to address this challenge. Unlike previous methods which rely on introducing learning modules to improve concept embeddings, our method directly optimize concept embeddings with respect to the training loss by injecting differentiability into the model. To maintain interpretability, we restrict the parameter space for concept embeddings to a small neighborhood around its initialization and the radius of the search space become an easy-to-tune parameter that controls the trade-off between performance and interpretability. To investigate the theoretical necessity and guarantees of our method, we follow the theoretical framework proposed in \cite{chattopadhyay2024information}, where concepts are regarded as queries being checked to predict a target random variable. Specifically, we make the following contributions:

\textbf{Theoretical Necessity.} To motivate our algorithm from a theoretical perspective, we first show that under the framework introduced by \cite{chattopadhyay2024information}, whenever there exists deviation between the concepts used in the learning algorithms and the concepts used to generate the data, there is a worst case lower bound for the performance of the algorithm (\Cref{theorem: formal necessity}). This result can be regarded as a theoretical evidence for the performance degradation caused by inaccurate concept embeddings.

\textbf{Convergence Guarantees.} Under the same setting as in \Cref{theorem: formal necessity}, we show that our framework \textit{Constrained Concept Refinement} effectively eliminate the performance degradation. Specifically, we prove that under the assumption that the target random variable can be perfectly explained by independent concepts, our algorithm achieve a population loss converging to zero (\Cref{theorem: vanishing L convergence}). Furthermore, under the condition that we are given enough training data, our algorithm provably recovers the ground truth concept embeddings used to generate the data (\Cref{theorem: columnwise convergence}). The results of both \Cref{theorem: vanishing L convergence} and \Cref{theorem: columnwise convergence} are verified by numerical tests.

\textbf{Real Experiments.} The framework studied in \Cref{theorem: vanishing L convergence} and \Cref{theorem: columnwise convergence} can be easily extended to solve real life problems like image classification. We run our algorithm on five different image classification benchmarks and see a clear spike on the test accuracy compared with the same model without \textit{Constrained Concept Refinement}. The experiments also show that our method is not only competitive with existing explainability methods but also computationally less expensive. Finally, we validate that our algorithm indeed effectively preserve interpretability. 

\subsection{Notations}
For a matrix $\rmA$, we use $\|\rmA\|_2$, $\|\rmA\|_F$, $\|\rmA\|_{1,2}$ to denote its spectral norm, Frobenius norm, the maximum of its column-wise 2-norm respectively. We define $[n] = \{1,2,\dots, n\}$. Given two sequences $f(n)$ and $g(n)$, the notations $f(n)=O(g(n))$ implies that there exists a universal constant $C>0$ satisfying $f(n) \leq Cg(n)$ for large enough $n$. $f(n)=\Omega(g(n))$ implies that for any real constant $c>0$, $f(n)>c g(n)$ for large enough $n$. We have $f(n)=o(g(n))$ if $\lim_{h\rightarrow\infty} f(n)/g(n) = \infty$. We claim an event happen with high probability if it happens with probability at least $1-n^{-\omega(1)}$ where $n$ is the number of concepts in the problem.


\subsection{Organization}
We will first provide a literature review in \Cref{section: review} to complement our introduction. We will introduce our main theoretical results in \Cref{section: theory}, which starts by introducing the problem setting and a classic greedy algorithm (\Cref{subsection: setup}). Then we will demonstrate that the classic method will face performance degradation when concept embeddings have deviation(\Cref{subsection: motivation}). In \Cref{subsection: convergence} we will show that our algorithm will provably resolve the issue. Finally, we will present our numerical experiments in \Cref{section: experiments} which contains both the experiments for synthetic datasets (\Cref{subsection: synthetic datasets}) to support results in \Cref{section: theory} and real datasets.

==> main_text/proof_2.tex <==
To prove the convergence of $\cL\bigbracket{\tf_{\mD^{(t)}}}$, we use an inductive approach where at each iteration, we will subsequently prove: (1) $\tf$ recovers the exact support $S^*$; (2) gradient descent will make progress towards one of the optimal minimizers which will be explicitly defined later; (3) $\cL\bigbracket{\tf_{\mD^{(t)}}}$ will decrease linearly. 

Recall that $\mD^{(t)} = \mD+\Delta\mD^{(t)}$. The equations below rewrite \Cref{eq: update rule} for each column $i\in [n]$ of $\mD^{(t)}$. 
\begin{align}
    \rvd^{(t+0.5)}_i &= \rvd^{(t)}_i - \eta\frac{\partial\cL(\tf_{\mD^{(t)}})}{\partial \rvd_i^{(t)}}, \label{eq: gd step}\\
    \rvd^{(t+1)}_i &= \argmin_{\rvd:\|\rvd - \rvd^{(0)}_i\|_2\le \rho} \|\rvd - \rvd^{(t+0.5)}_i\|_2. \label{eq: projection step}
\end{align}
It is easy to verify that the above update rules are equivalent to \Cref{eq: update rule}.
We will use induction to prove this theorem. In particular, define
\begin{align*}
    % A(t):&\quad \hrvd_i - \rvd^{(t)}_i = \frac{\beta_i - \rvx^\top\rvd^{(t)}_i}{\|\rvx\|^2_2}\rvx,\\
    A(t):&\quad \cL(\tf_{\mD^{(t)}})\le \tau^2 \cL(\tf_{\mD^{(t-1)}}).
    % \|\hrvd_i - \rvd^{(t+1)}_i \|_2 \le \tau \|\hrvd_i - \rvd^{(t)}_i \|_2.
\end{align*}
To prove this we define an auxiliary feature vector which will play an important role in our arguments:
\begin{align}\label{eq: hat d definition}
    \hrvd_i = \rvd^{(0)}_i + \frac{\beta_i - \rvx^\top\rvd^{(0)}_i}{\|\rvx\|^2_2}\rvx, \qquad \forall i\in S^*.
\end{align}
Based on this auxiliary feature vector, we define the following event:
% We will use a mathematical induction approach and our induction hypothesis are:
\begin{align*}
    B(t):&\quad \hrvd_i - \rvd^{(t)}_i = \frac{\beta_i - \rvx^\top\rvd^{(t)}_i}{\|\rvx\|^2_2}\rvx, \qquad \forall i\in S^*.
    % B(t):&\quad \cL(\tf_{\mD^{(t)}})\le \tau^2 \cL(\tf_{\mD^{(t-1)}}).
    % \|\hrvd_i - \rvd^{(t+1)}_i \|_2 \le \tau \|\hrvd_i - \rvd^{(t)}_i \|_2.
\end{align*}
Now, our proof strategy is to show that, for $t=0,1,\dots$:
\begin{itemize}
    \item $B(t)$ implies $B(t+1)$,
    \item $B(t)$ implies $A(t+1)$.
\end{itemize}
This two statements combined will establish the correctness of \Cref{theorem: vanishing L convergence}
% $B(t)$ implies $A(t+1)$, and $B(t)$ implies $B(t+1)$. 
% We will show for some $t$, $A(t)\rightarrow A(t+1)$ and $A(t)\rightarrow B(t+1)$, which will essentially prove \Cref{theorem: vanishing L convergence}. 
Indeed, the base case $A(0)$ is trivially satisfied due to \Cref{eq: hat d definition}.

To begin with, we use the following lemma to show that $\tf$ is able to find the correct support when $\mD^{(t)}$ is close enough to $\mD$: 
\begin{lemma}\label{lemma: support recovery}
    For any $\mD$ such that $\|\mD-\mD^*\|_{1,2}\le2\rho<\frac{1}{4}$, with probability at least $1 - 2 \exp\left\{\log n-\frac{\gamma^2}{128\rho^2\sigma^2}\right\}$, we have 
    \begin{align*}
        S = \argmax_{T \subseteq [n], |T| \le k} \sum_{i \in T} |\langle \rvd_i, \rvx \rangle| = S^*.
    \end{align*}
\end{lemma}
We defer the proof of \Cref{lemma: support recovery} to \Cref{section: proof to lemma support recovery}. To invoke \Cref{lemma: support recovery}, we have
\begin{align*}
    \|\mD^{(t)} - \mD^*\|_{1,2} \le \|\mD^{(t)} - \mD^{(0)}\|_{1,2} + \|\mD^{(0)} - \mD^*\|_{1,2} \le \rho + \rho = 2\rho.
\end{align*}
The bound on $\|\mD^{(t)} - \mD^{(0)}\|_{1,2}$ comes from the projection step \Cref{eq: projection step} while the bound on $\|\mD^{(0)} - \mD^*\|_{1,2} $ follows from the initial error bound. We can then conclude that $S=S^*$ at $t$th iteration, which means that \Cref{eq: gd step} and \Cref{eq: projection step} will only apply to $i\in S^*$ while for other $i\not\in S^*$, $\rvd^{(t+1)}_i = \rvd^{(t)}_i$. 

Based on \Cref{eq: def L f_D part 1} and \Cref{eq: def L f_D part 2}, we have
\begin{align*}
    \cL(\tf_{\mD^{(t)}}) = \|\mD^*_{S^*}\mD^{(t)\top}_{S^*} \rvx -\rvx\|^2_2,
\end{align*}
Subsequently, we have the gradient for $\mD^{(t)}_{S^*}$ defined as:
\begin{align*}
    \frac{\partial\cL(\tf_{\mD^{(t)}})}{\partial \mD^{(t)}_{S^*}} &= 2\rvx\bigbracket{\mD^*_{S^*}\mD^{(t)\top}_{S^*} \rvx -\rvx}^\top \mD^*_{S^*}\\
    &=2\rvx\bigbracket{\mD^*_{S^*}\mD^{(t)\top}_{S^*} \rvx -\mD^*_{S^*}\rvbeta_{S^*}}^\top \mD^*_{S^*}\\
    &= 2\rvx\bigbracket{\mD^{(t)\top}_{S^*} \rvx -\rvbeta_{S^*}}^\top \mD^{*\top}_{S^*}\mD^*_{S^*}\\
    &= 2\rvx\bigbracket{\mD^{(t)\top}_{S^*} \rvx -\rvbeta_{S^*}}^\top.
\end{align*}
For $i\in S^*$, we have
\begin{align*}
    \frac{\partial\cL(\tf_{\mD^{(t)}})}{\partial \rvd^{(t)}_i} = 2(\rvd^{(t)\top}_i\rvx - \rvbeta_i)\rvx.
\end{align*}
We are ready to show $A(t+0.5)$:
\begin{align*}
    \hrvd_i - \rvd^{(t+0.5)}_i &= \hrvd_i - \rvd^{(t)}_i + 2\eta (\rvd^{(t)\top}_i\rvx - \rvbeta_i)\rvx \\
    &\overset{A(t)}{=}\frac{\beta_i - \rvx^\top\rvd^{(t)}_i}{\|\rvx\|^2_2}\rvx+ 2\eta (\rvd^{(t)\top}_i\rvx - \rvbeta_i)\rvx \\
    &=\frac{\beta_i - \rvx^\top\bigbracket{\rvd^{(t+0.5)}_i+2\eta (\rvd^{(t)\top}_i\rvx - \rvbeta_i)\rvx}}{\|\rvx\|^2_2}\rvx+ 2\eta (\rvd^{(t)\top}_i\rvx - \rvbeta_i)\rvx \\
    &= \frac{\beta_i - \rvx^\top\rvd^{(t+0.5)}_i}{\|\rvx\|^2_2}\rvx - 2\eta (\rvd^{(t)\top}_i\rvx - \rvbeta_i)\rvx +2\eta (\rvd^{(t)\top}_i\rvx - \rvbeta_i)\rvx \\
    &= \frac{\beta_i - \rvx^\top\rvd^{(t+0.5)}_i}{\|\rvx\|^2_2}\rvx.
\end{align*}
Next, we aim to show that $\|\hrvd_i - \rvd^{(t+0.5)}_i\|_2\le \tau\|\hrvd_i - \rvd^{(t)}_i\|_2$. Specifically, we can show that:
\begin{align*}
    \|\hrvd_i - \rvd^{(t+0.5)}_i\|_2 &= 
    \|\hrvd_i - \rvd^{(t)}_i+ 2\eta (\rvd^{(t)\top}_i\rvx - \rvbeta_i)\rvx\|_2\\
    &\overset{A(t)}{=} 
    \left\|\hrvd_i - \rvd^{(t)}_i- 2\eta \|\rvx\|^2_2\bigbracket{\hrvd_i - \rvd^{(t)}_i} \right\|_2\\
    &\le \left|1-2\eta\|\rvx\|^2_2\right|\|\hrvd_i - \rvd^{(t)}_i\|_2\\
    &= \tau\|\hrvd_i - \rvd^{(t)}_i\|_2.
\end{align*}
Suppose $\|\rvd^{(t+0.5)}_i - \rvd^{(0)}_i\|_2\le\rho$, then we have $\rvd^{(t)}_i = \rvd^{(t+0.5)}_i$, which directly leads to $A(t+1)$ and $\|\hrvd_i - \rvd^{(t+1)}_i\|_2\le \tau\|\hrvd_i - \rvd^{(t)}_i\|_2$. If $\|\rvd^{(t+0.5)}_i - \rvd^{(0)}_i\|_2>\rho$, we have:
\begin{equation}\label{eq: d^(t+0.5) - d^(0)}
    \begin{aligned}
    \rvd^{(t+0.5)}_i - \rvd^{(0)}_i
    &= \bigbracket{\rvd^{(t+0.5)}_i-\hrvd_i } - \bigbracket{\rvd^{(0)}_i-\hrvd_i } \\
    &\overset{A(t+0.5),A(0)}{=} -\frac{\beta_i - \rvx^\top\rvd^{(t+0.5)}_i}{\|\rvx\|^2_2}\rvx + \frac{\beta_i - \rvx^\top\rvd^{(0)}_i}{\|\rvx\|^2_2}\rvx \\
    &=  \frac{\rvx^\top\rvd^{(t+0.5)}_i - \rvx^\top\rvd^{(0)}_i}{\|\rvx\|^2_2}\rvx,
\end{aligned}
\end{equation}

So we have when $\|\rvd^{(t+0.5)}_i - \rvd^{(0)}_i\|_2>\rho$:
\begin{equation}\label{eq: d^(t+1) definition}
    \begin{aligned}
    \rvd^{(t+1)}_i & = \argmin_{\rvd:\|\rvd - \rvd^{(0)}_i\|_2\le \rho} \|\rvd - \rvd^{(t+0.5)}_i\|_2 \\
    &= \rvd^{(0)}_i + \rho\frac{\rvd^{(t+0.5)}_i - \rvd^{(0)}_i}{\|\rvd^{(t+0.5)}_i - \rvd^{(0)}_i\|_2}\\
    &= \rvd^{(0)}_i + \rho\sign\bigbracket{\rvx^\top\rvd^{(t+0.5)}_i - \rvx^\top\rvd^{(0)}_i}\frac{\rvx}{\|\rvx\|_2}.
\end{aligned}
\end{equation}

We are then ready to show $A(t+1)$ when $\|\rvd^{(t+0.5)}_i - \rvd^{(0)}_i\|_2>\rho$:
\begin{align*}
    &\quad \ \hrvd_i - \rvd^{(t+1)}_i \\
    &= \hrvd_i - \rvd^{(0)}_i - \rho\sign\bigbracket{\rvx^\top\rvd^{(t+0.5)}_i - \rvx^\top\rvd^{(0)}_i}\frac{\rvx}{\|\rvx\|_2} \\
    &\overset{A(0)}{=}\frac{\beta_i - \rvx^\top\rvd^{(0)}_i}{\|\rvx\|^2_2}\rvx - \rho\sign\bigbracket{\rvx^\top\rvd^{(t+0.5)}_i - \rvx^\top\rvd^{(0)}_i}\frac{\rvx}{\|\rvx\|_2}\\
    &=\frac{\beta_i - \rvx^\top\bigbracket{\rvd^{(t+1)}_i-\rho\sign\bigbracket{\rvx^\top\rvd^{(t+0.5)}_i - \rvx^\top\rvd^{(0)}_i}\frac{\rvx}{\|\rvx\|_2}}}{\|\rvx\|^2_2}\rvx-\rho\sign\bigbracket{\rvx^\top\rvd^{(t+0.5)}_i - \rvx^\top\rvd^{(0)}_i}\frac{\rvx}{\|\rvx\|_2} \\
    &= \frac{\beta_i - \rvx^\top\rvd^{(t+1)}_i}{\|\rvx\|^2_2}\rvx.
\end{align*}
Up to now, we have proved $A(t+1)$. Next, we try to show $\|\hrvd_i - \rvd^{(t+1)}_i\|_2\le \tau\|\hrvd_i - \rvd^{(t)}_i\|_2$ by showing $\|\hrvd_i - \rvd^{(t+1)}_i\|_2\le \|\hrvd_i - \rvd^{(t+0.5)}_i\|_2$. To do so, we need the following elementary lemma:
\begin{lemma}\label{lemma: elementary position}
    Given a fixed vector $\rvv$ and $\rva = a\rvv$, $\rvb = b\rvv$, $\rvc = c\rvv$, where $\rva$, $\rvb$ and $\rvc$ are vectors and $a$, $b$, $c$ are scalars, if $|c|\ge|b|\ge a$ and $bc>0$, we have $\|\rvc-\rva\|_2\ge \|\rvb-\rva\|_2$.
\end{lemma}
We will prove \Cref{lemma: elementary position} in \Cref{section: proof to lemma elementary position}. Now we invoke \Cref{lemma: elementary position} with:
\begin{align*}
    \rvv &= \frac{\rvx}{\|\rvx\|_2},\\
    a &= \frac{\rvbeta_i - \rvx^\top\rvd^{(0)}_i}{\|\rvx\|_2},\\
    b &= \rho \sign\bigbracket{\rvx^\top\rvd^{(t+0.5)}_i - \rvx^\top\rvd^{(0)}_i},\\
    c &= \frac{\rvx^\top\rvd^{(t+0.5)}_i - \rvx^\top\rvd^{(0)}_i}{\|\rvx\|_2}.
\end{align*}
Here $bc>0$ is given by their definition. $|c|\ge|b|$ is given by:
\begin{align*}
    |c|=& \left|\frac{\rvx^\top\rvd^{(t+0.5)}_i - \rvx^\top\rvd^{(0)}_i}{\|\rvx\|_2}\right| \\
    =& \left\| \frac{\rvx^\top\rvd^{(t+0.5)}_i - \rvx^\top\rvd^{(0)}_i}{\|\rvx\|^2_2}\rvx \right\|_2 \\
    \overset{Eq\ref{eq: d^(t+0.5) - d^(0)}}{=}&\|\rvd^{(t+0.5)}_i - \rvd^{(0)}_i\|_2 \\
    \ge & \rho \\
    = & |b|.
\end{align*}
$|b|>a$ is given by:
\begin{equation}\label{eq: a<b}
    \begin{aligned}
    a &= \frac{\rvbeta_i - \rvx^\top\rvd^{(0)}_i}{\|\rvx\|_2}\\
    &=\frac{\rvx^\top\rvd^*_i - \rvx^\top\rvd^{(0)}_i}{\|\rvx\|_2} \\
    &\le \frac{\|\rvd^*_i-\rvd^{(0)}_i\|_2\|\rvx\|_2}{\|\rvx\|_2}\\
    &\le \|\rmD^*-\rmD^{(0)}\|_{1,2} \\
    &= \rho \\
    &= |b|.
\end{aligned}
\end{equation}

Now, after plugging everything into the conclusion of \Cref{lemma: elementary position}, we have:
\begin{align*}
    \|\rvc-\rva\|_2 &\ge \|\rvb-\rva\|_2 \\
    \left\|\frac{\rvx^\top\rvd^{(t+0.5)}_i - \rvx^\top\rvd^{(0)}_i}{\|\rvx\|^2_2}\rvx - \frac{\beta_i - \rvx^\top\rvd^{(0)}_i}{\|\rvx\|^2_2}\rvx\right\|_2 &\ge \left\|\rho \sign\bigbracket{\rvx^\top\rvd^{(t+0.5)}_i - \rvx^\top\rvd^{(0)}_i}\frac{\rvx}{\|\rvx\|_2}- \frac{\beta_i - \rvx^\top\rvd^{(0)}_i}{\|\rvx\|^2_2}\rvx\right\|_2\\
    \left\|\bigbracket{\rvd^{(t+0.5)}_i - \rvd^{(0)}_i}-\bigbracket{\hrvd_i-\rvd^{(0)}_i}\right\|_2&\overset{(a)}{\ge}\left\|\bigbracket{\rvd^{(t+1)}_i - \rvd^{(0)}_i}-\bigbracket{\hrvd_i-\rvd^{(0)}_i}\right\|_2\\
    \|\rvd^{(t+0.5)}_i-\hrvd_i\|_2 &\ge \|\rvd^{(t+1)}_i-\hrvd_i\|_2
\end{align*}
Here inequality (a) is given by \Cref{eq: d^(t+0.5) - d^(0)}, \Cref{eq: hat d definition} and \Cref{eq: d^(t+1) definition}. We can now conclude that:
\begin{align}\label{eq: d^(t+1) < d^(t)}
    \|\rvd^{(t+1)}_i-\hrvd_i\|_2 \le \|\rvd^{(t+0.5)}_i-\hrvd_i\|_2 \le \tau \|\rvd^{(t)}_i-\hrvd_i\|_2.
\end{align}
Finally, we are ready to prove $B(t+1)$. We rewrite $\cL(\tf_{\mD^{(t)}})$ as:
\begin{align*}
    \cL(\tf_{\mD^{(t)}}) & = \|\mD^*_{S^*}\mD^{(t)\top}_{S^*} \rvx -\rvx\|^2_2 \\
    &= \|\mD^*_{S^*}\mD^{(t)\top}_{S^*} \rvx -\mD^*_{S^*}\rvbeta_{S^*}\|^2_2 \\
    &= \|\mD^{(t)\top}_{S^*} \rvx -\rvbeta_{S^*}\|^2_2\\
    &= \sum_{i\in S^*} \bigbracket{\rvx^\top\rvd^{(t)}_i-\rvbeta_i}^2 \\
    &= \sum_{i\in S^*}\left\|\frac{\beta_i - \rvx^\top\rvd^{(t)}_i}{\|\rvx\|^2_2}\rvx\right\|^2_2 \|\rvx\|^2_2\\
    &\overset{A(t)}{=}\sum_{i\in S^*}\left\|\rvd^{(t)}_i-\hrvd_i\right\|^2_2 \|\rvx\|^2_2
\end{align*}
Since we also have $A(t+1)$, we have 
\begin{align*}
    \cL(\tf_{\mD^{(t+1)}}) = \sum_{i\in S^*}\left\|\rvd^{(t+1)}_i-\hrvd_i\right\|^2_2 \|\rvx\|^2_2
\end{align*}
by identical arguments. Finally, we have
\begin{align*}
    \cL(\tf_{\mD^{(t+1)}}) = \sum_{i\in S^*}\left\|\rvd^{(t+1)}_i-\hrvd_i\right\|^2_2 \|\rvx\|^2_2 \overset{Eq\ref{eq: d^(t+1) < d^(t)}}{\le} \tau^2\sum_{i\in S^*}\left\|\rvd^{(t)}_i-\hrvd_i\right\|^2_2 \|\rvx\|^2_2 = \cL(\tf_{\mD^{(t)}}),
\end{align*}
which is exactly $B(t+1)$. As a result, we have proved the linear convergence statement of \Cref{theorem: vanishing L convergence}. Finally, we need to provide a lower bound for the probability that this convergence result happens, which depends on the number of times we invoke \Cref{lemma: support recovery}. For a total of $T$ iterations, the result will hold with probability at least $1 - 2T\exp\left\{\log n-\frac{\gamma^2}{128\rho^2\sigma^2}\right\}$. When $T\rightarrow \infty$, we cannot claim \Cref{theorem: vanishing L convergence} holds with high probability. Here we use the following lemma to avoid repeatedly invoking \Cref{lemma: support recovery} when $\rvd^{(0)}_i$ is close enough to $\hrvd_i$. 
\begin{lemma}\label{lemma: support recovery around hrvd}
    Denote $\widehat{\mD} = \begin{bmatrix}
        \hrvd_1,...,\hrvd
    \end{bmatrix}$ where $\hrvd_i$ is defined in \Cref{eq: hat d definition} for $i\in S^*$ and $\hrvd_i=\rvd^{(0)}_i$ for $i\not\in S^*$, with probability at least $1 - 2 \exp\left\{\log n-\frac{\gamma^2}{512\rho^2\sigma^2}\right\}$, we have
    \begin{align*}
        S = \argmax_{T \subseteq [n], |T| \le k} \sum_{i \in T} |\langle \rvd_i, \rvx \rangle| = S^*.
    \end{align*}
    for all $\mD$ such that $\|\mD-\mD^*\|_{1,2}\le2\rho<\frac{1}{4}$ and $\|\mD-\widehat{\mD}\|_{1,2}\le \frac{\gamma}{8k\Gamma}$.
\end{lemma}
Our strategy to bound the probability that support recovery happens for every iteration is as follows: (1) when $\|\mD^{(t)}-\widehat{\mD}\|_{1,2}> \frac{\gamma}{8k\Gamma}$, we invoke $\Cref{lemma: support recovery}$ for every iteration. Since \Cref{eq: d^(t+1) < d^(t)} shows that columns in $S^*$ converge to $\hrvd_i$ linearly in this situation, we only need to invoke $\Cref{lemma: support recovery}$ for a total of $\log_\tau\bigbracket{\frac{\rho}{\gamma/8k\Gamma}} = \log_\tau (8k\Gamma\rho/\gamma)$ times; (2) after $\|\mD^{(t)}-\widehat{\mD}\|_{1,2}\le \frac{\gamma}{8k\Gamma}$ \Cref{eq: d^(t+1) < d^(t)} shows that the iterate will always be close to $\widehat{\mD}$ and we only need to invoke \Cref{lemma: support recovery around hrvd} once. In total, exact support recovery for every iteration happens with probability at least $1-2\log_\tau (8k\Gamma\rho/\gamma)\exp\left\{\log n-\frac{\gamma^2}{128\rho^2\sigma^2}\right\} - 2 \exp\left\{\log n-\frac{\gamma^2}{512\rho^2\sigma^2}\right\}$, which is $1-n^{-\omega(1)}$ when $\rho = O\left(\frac{1}{\log n}\right)$. The proof to \Cref{theorem: vanishing L convergence} is complete.
